Geometric interpretation of the vanishing Lie Bracket for two-dimensional rough vector fields

In this paper, we prove that if $X,Y$ are continuous, Sobolev vector fields with bounded divergence on the real plane and $[X,Y]=0$, then their flows commute. In particular, we improve the previous result of Colombo-Tione (2021), where the authors require the additional assumption of the weak Lie differentiability on one of the two flows. We also discuss possible extensions to the $\text{BV}$ setting.

==> appunti.tex <==
\begin{theorem}\label{thm:comm-BV}
 Let $X$, $Y \in \BV_{\text{loc}}(\R^n,\R^n)\cap L^\infty(\R^n,\R^n)$ be vector fields with bounded divergence and let $\phi_t^X$, $\phi_s^Y$ be their Regular Lagrangian Flows. Then the two following statements are equivalent:
 \begin{itemize}
     \item[(i)] the flows of $X$ and $Y$ commute;
     \item[(ii)]  the Lie bracket $[X,Y]$ is $0$ and $\phi^X_t$ is weakly (Lie) differentiable in direction $Y$ with locally bounded derivative. Moreover {\color{red} qua condizione aggiuntiva + forse dobbiamo richiedere che i cambi abbiano divergenza nulla?}
 \end{itemize}
\end{theorem}
As already pointed out, Theorem \ref{thm:comm-BV} generalizes the analogous result for Sobolev vector fields obtained in \cite{ColomboTione}. However, our result does not follow straightforwardly from the Sobolev case, as it requires a refined analysis of the difference quotients of $\BV$ functions in the spirit of what has been performed in \cite{Ambrosio:BV}. In particular we observe that, if $\phi^X_t\in\BV$ {\color{red} vale la weakly lie differentiability? o va definita in modo diverso?}.

We are now in a position to carry out the proof of one of our main results, Theorem \ref{thm:comm-BV}.

\medskip
\noindent
\textit{Proof of Theorem \ref{thm:comm-BV}.} In virtue of Proposition \ref{prop:commutativity}, we only need to prove the missing implication, namely that $[X,Y]\equiv 0$ implies that $T_t \equiv 0$ under the additional assumption on the differentiability of flow of one vector field in the direction of the other vector field. We first observe that the flow of $Y$ is weakly (Lie) differentiable along $Y$ and its derivative is equal to $Y \circ \phi_s^Y$, namely
 \begin{equation*}
    \int_{R^n}\left(\phi_s^Y(z),D\varphi(z) Y(z)\right)+\dive(Y)(z)\left(\phi_s^Y(z),\varphi(z)\right)dz=-\int_{\R^n}\left(Y(\phi_s^Y(z)),\varphi(z)\right)dz, \quad  \forall s \in \R.
    \end{equation*}
    Then the previous equation for $s=0$ yields $T_0=0$. We now aim at showing that $[X,Y](\phi_t^X)=0$ in the sense of Definition \ref{def:Lie-bracket-flow} implies $   \frac{d}{dt} T_t[X,Y](\varphi)=0$. We first rewrite condition $[X,Y](\phi_t^X)=0$ as follows
\begin{equation}\label{eq:zero-dist-lie-bracket}
 \int_{\R^n} ([X,Y](\phi_t^X),\varphi) dz   = \int_{\R^n}\left(X,D \varphi \circ \phi_{-t}^X D\phi_{-t}^X Y\right)\xi(-t,z)dz-\int_{\R^n}\left(Y,D \varphi \circ \phi_{-t}^X D\phi_{-t}^X X\right)\xi(-t,z)dz=0.
\end{equation}
Reasoning as above and performing the change of variable $\tilde{z}=\phi^X_{-t}(z)$, we can rewrite equation \eqref{eq:zero-dist-lie-bracket} as
\begin{equation}\label{eq:zero-distr-lie-bracket-2}
 \int_{\R^n}\left(X(\phi_{t}^X(\tilde z)),D \varphi (\tilde z)D\phi_{-t}^X Y(\phi_{t}^X(\tilde z)\right)d  \tilde z-\int_{\R^n}\left(Y(\phi_{t}^X(\tilde z),D \varphi (\tilde z) X(\tilde z)\right)d\tilde z=0.
\end{equation}
Owing to \eqref{eq:der-distr} with $\dive X= \dive Y=0$, it is clear that \eqref{eq:zero-distr-lie-bracket-2} implies $   \frac{d}{dt} T_t[X,Y](\varphi)=0$ if and only if
\begin{equation*}
    \int_{\R^n}\left(X(\phi_{t}^X),D \varphi D\phi_{-t}^X Y(\phi_{t}^X)\right)dz =\int_{\R^n}(X (\phi_t^X), D\varphi Y)dz.
\end{equation*}
{\color{red}Mi inquieta molto questa parte}

$\hfill \square$



\begin{remark}\label{rmk:flow:diff:in:its:direct}
    We remark that if $X\in \BV_{\text{loc}}(\R^d,\R^d)$ with $\dive X\in L^\infty(\R^d,\R)$, then $\phi^X_t$ is weakly (Lie) differentiable w.r.t. $X$, for every time $t$. This is an easy consequence of the fact that $[X,X]=0$, which implies, thanks to the previous computations, $T_t[X,X]=0$ for every time $t$. 
\end{remark}


 For this reason, we provide the following definition for divergence-free vector fields.
\begin{definition}\label{def:Lie-bracket-flow}
Let $X$, $Y \in \BV_{\text{loc}}(\R^n,\R^n)\cap L^\infty(\R^n,\R^n)$ be divergence-free vector fields. Then we define the (distributional) Lie bracket $[X,Y]$ along the flow $\phi_t^X$ by setting
\begin{equation}\label{eq:def:lie:brack:flow}
    \int_{\R^n} ([X,Y](\phi_t^X),\varphi) dz \doteq  \int_{\R^n} ([X,Y],\varphi \circ \phi_{-t}^X) \xi(-t,z) dz,  \qquad  \forall \varphi\in C^1_c(\R^n,\R^n),
\end{equation}
where $\xi$ denotes the density associated to the “change of variables” identity in \eqref{eq:change-of-var}.
\end{definition}
We remark that Definition \ref{def:Lie-bracket-flow} seems to be the most natural one in this context, since it is obtained by testing equation \eqref{eq:def:lie:brack} against the funcion $\varphi \circ \phi_{-t}^X$ (this choice of the test function can be made rigorous by mollifying $\left(\varphi \circ \phi_{-t}^X\right) \ast \rho_\epsilon$ and then by passing to the limit as $\epsilon \to 0$).

{\color{red}Motivare questa definizione. Vale la pena mettere qui la strategia della dimostrazione del Teorema 1.3?}
{\color{red} decidere come fare questo? se mettere solo un campo sobolev}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Caso non continuo

We point out that the non-continuous case, though solvable if $X\cdot Y^\perp=0$ (see Subsection \ref{ss:non:continuous}), would require different ideas in the case $X\cdot Y^\perp=1$. We expect that, by carefully adapting the ideas in \cite{Eliodiff}, one should conclude the same results also under the non-continuity assumption.

%\begin{remark}
  %  In the next subsection we will prove the same results, dropping the continuity assumption on the two vector fields $X$ and $Y$. Clearly, we cannot expect the commutativity of flows in the sense of Equation \eqref{eq:strong:commutativity}, but the weaker one that has been assumed throughout the paper. 
%\end{remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align*}
    \int_{\R^2}(X,D\varphi Y)-(Y,D\varphi X)dz&=\int_{\R^2}(\nabla^\perp H,D\varphi \nabla^\perp K)-(\nabla^\perp K,D\varphi \nabla^\perp H)dz.
\end{align*}
In particular, 
\begin{align*}
    \int_{\R^2}(\nabla^\perp H,D\varphi \nabla^\perp K)dz &=\int_{\R^2} \left(\partial_2H\partial_2K\partial_1\varphi_1-\partial_2H\partial_1K\partial_2\varphi_1 -\partial_1 H\partial_2 K\partial_1\varphi_2+\partial_1 H\partial_1K\partial_2\varphi_2 \right) dz,
\end{align*}
so that
\begin{align*}
    &\int_{\R^2}(\nabla^\perp H,D\varphi \nabla^\perp K)-(\nabla^\perp K,D\varphi \nabla^\perp H)dz= \\&\int_{\R^2} (-\partial_2H\partial_1K\partial_2\varphi_1 -\partial_1 H\partial_2 K\partial_1\varphi_2+\partial_2 K\partial_1H\partial_2\varphi_1+\partial_1K\partial_2H\partial_1\varphi_2)dz=\\& \int_{\R^2} (\nabla^\perp H, \nabla K)\partial_2\varphi_1 +(\nabla^\perp K,\nabla H)\partial_1\varphi_2 dz=\\&-\int_{\R^2} X\cdot Y^\perp(\partial_2\varphi_1-\partial_1\varphi_2)dz,
\end{align*}
which gives the statement.
In the general case,
\begin{align*}
    \int_{\R^2}(X,D\varphi Y)-(Y,D\varphi X)dz&=\int_{\R^2}(Y_1X_1\partial_1\varphi_1+X_1Y_2\partial_2\varphi_1+ Y_1X_2\partial_1\varphi_2+Y_2X_2\partial_2\varphi_2)dz.
\end{align*}
\end{proof}
\begin{remark}
    We observe that Equation \eqref{eq:Lie:bracket} and Lemma \ref{lem:eq:for:bracket} hold also in the $\BV$ setting.
\end{remark}

==> wld.tex <==
\section{Remarks on the weak Lie differentiability}
As anticipated in the introduction, we want to give some insights on the condition of weakly Lie differentiability. 
We have the following
\begin{proposition}
Let $X,Y\in W^{1,p}_{\text{loc}}(\R^2,\R^2)\cap L^\infty(\R^2,\R^2)$ with bounded divergence. Assume that $X,Y$ are \emph{linearly independent} a.e., that is there exist functions $\alpha_1,\beta_1,\alpha_2,\beta_2\in W^{1,p}_{\text{loc}}(\R^2,\R)\cap L^\infty(\R^2,\R)$ with the property that
\begin{equation}\label{eq:lin:indep}
    e_i=\alpha_iX+\beta_i Y \text{ a.e., }\quad i=1,2,
\end{equation}
where $e_1,e_2$ denote the vectors of the canonical base. Then
\begin{equation*}
    \phi^X_t \text{ is weakly (Lie) differentiable w.r.t. } Y \iff \phi^X_t\in W^{1,p}_{\text{loc}}(\R^2).
\end{equation*}
\end{proposition}
\begin{remark}
    This proposition tells us that the weak derivative of $\phi^X_t$ is a directional derivative. 
\end{remark}
\begin{proof}
    We start with the following observation: $\phi^X_t$ is weakly (Lie) differentiable w.r.t. $X$. This is an easy consequence of the fact that $[X,X]=0$, which distributionally reads as
    \begin{equation*}
        \int_{R^n}\left(\phi^X_t(z),D\varphi(z) X(z)\right)+\dive(X)(z)\left(\phi^X_t(z),\varphi(z)\right)dz=-\int_{\R^n}\left(X(\phi^X_t(z)),\varphi(z)\right)dz,
    \end{equation*}
    (see Remark \ref{rmk:flow:diff:in:its:direct}).
    
\end{proof}
\begin{remark}
    Is there some further regularity? So if I assume X,Y linearly independent a.e. does this mean that there is some continuity or the fact that they do not get to zero too badly? Secondo me è una domanda interessante.
\end{remark}

For the first case we have just shown the commutation of the flows, while in the second case we have that $X,Y$ are linearly independent a.e. 
{\color{red} Qui ci vuole la cosa di Elio } this in particular extends the corollary of [Colombo, Tione]. Indeed we have

%\begin{proposition} Voglio girare al negativo la proposizione di Elio. Come devo fare? Dal suo esempio pero` sembrerebbe che il campo e` sempre positivo, anche se Alberti etc trovano altro onestamente.. e lui non fa sto conto. 
 %   Let $X\in \BV(\R^2,\R^2)$ be a divergence-free vector field. If there exists $\bar t$, $\Omega'\subset \R^2$ open set such that $\phi^X_{\bar t} \not\in \BV(\Omega')$ then there exists $\Omega\supset\Omega'$ such that $X=0$ a.e. in $\Omega$. 
%\end{proposition}
\begin{remark}
    We remark that in order to prove that the Lie-differentiability is necessary (in the divergence-free setting) we need to find $X, Y$ such that $X\cdot Y^\perp=1$ a.e. such that there exists $\bar t$ with $\phi^X_{\bar t}\not\in \BV_{\text{loc}}(\R^2)$ (or the other one). In particular, both $|X|,|Y|$ should be bounded from below a.e.. So we have that there exists a set $\Omega$ such that $\phi^X_{\bar t}\not\in \BV(\Omega)$. This forces $\phi^Y_{\bar t}\in \BV(\Omega)$ thanks to the condition $X\cdot Y^\perp =1$. Therefore the search for counterexamples has to be done in the setting of [Marconi]. With this aim we found a well-known result in Hamiltonian Dynamics that states that, if $Y,Y^\perp$ such that $[Y,Y^\perp]=0$, $d=2$, then $Y$ is analytic. In particular, $Y$ gains regularity thanks to the condition $[Y,Y^\perp]=0$. It would be particularly interesting to investigate if the condition $[X,Y]=0$ gives further regularity to vector fields.
\end{remark}


\begin{proposition}
    Let $X,Y\in W^{1,p}_{\text{loc}}(\R^d,\R^d)\cap L^\infty(\R^d,\R^d)$ with bounded divergence, and assume that there exists $\alpha\in W^{1,p}_{\text{loc}}(\R^d,\R)\cap L^\infty(\R^d,\R)$ such that $X=\alpha Y$. 
    Then $\phi^X_t\circ\phi_s^Y=\phi_s^Y\circ \phi^X_t$ a.e. $x$, for every $s,t$. 
\end{proposition}
\begin{proof}
    We prove that $\phi^X_t$ is weakly (Lie) differentiable w.r.t. $Y$ in $\R^d$. 
   
    
    We have that, for every $\phi\in C^1_c(\R^2,\R^2)$
    \begin{align*}
        &\int_{\R^d}\left(\phi^X_t,D\varphi Y\right)+\dive(Y)\left(\phi^X_t,\varphi\right)dz=\\&
        \int_{\R^d}\left(\phi^X_t,D\varphi (\alpha X)\right)+\dive(\alpha X)\left(\phi^X_t,\varphi\right)dz.
    \end{align*} 
   In particular, using a mollification of $\alpha$
   \begin{align*}
        &\int_{\R^d}\left(\phi^X_t,D\varphi (\alpha X)\right)+\dive(\alpha X)\left(\phi^X_t,\varphi\right)dz\\&=\int_{\R^d}\left(\phi^X_t,D(\varphi \alpha) X \right)+\dive(\alpha X)\left(\phi^X_t,\varphi\right)dz-\int_{\R^d}\left(\phi^X_t,\varphi\cdot\nabla\alpha X \right)dz\\ &=-\int_{\Omega_\ell}\left(X(\phi^X_t),\varphi \alpha\right)-\dive(X)\left(\phi^X_t,\alpha\varphi\right)+\dive(\alpha X)\left(\phi^X_t,\varphi\right)dz-\int_{\R^d}\left(\phi^X_t,\varphi\cdot\nabla\alpha X \right)dz.
    \end{align*} 
    Where we have used that $\phi^X_t$ is weakly Lie differentiable w.r.t. $X$ (see Remark \ref{rmk:flow:diff:in:its:direct}). 
\end{proof}

